Budget Constrained Interactive Search for Multiple Targets

Interactive graph search leverages human intelligence to categorize target labels in a hierarchy, which are useful for image classification, product categorization, and database search. However, many existing studies of interactive graph search aim at identifying a single target optimally, and suffer from the limitations of asking too many questions and not being able to handle multiple targets. To address these two limitations, in this paper, we study a new problem of budget constrained interactive graph search for multiple targets called kBM-IGS-problem. Specifically, given a set of multiple targets T in a hierarchy, and two parameters k and b, the goal is to identify a k-sized set of selections S such that the closeness between selections S and targets T is as small as possible, by asking at most a budget of b questions. We theoretically analyze the updating rules and design a penalty function to capture the closeness between selections and targets. To tackle the kBM-IGS-problem, we develop a novel framework to ask questions using the best vertex with the largest expected gain, which makes a balanced trade-off between target probability and benefit gain. Based on the kBM-IGS framework, we first propose an efficient algorithm STBIS to handle the SingleTarget problem, which is a special case of kBM-IGS. Then, we propose a dynamic programming based method kBM-DP to tackle the MultipleTargets problem. To further improve efficiency, we propose two heuristic but efficient algorithms kBM-Topk and kBM-DP+. kBM-Topk develops a variant gain function and selects the top-k vertices independently. kBM-DP+ uses an upper bound of gains and prunes disqualified vertices to save computations. Experiments on large real-world datasets with ground-truth targets verify both the effectiveness and efficiency of our proposed algorithms.

==> tex/algorithm.tex <==
\section{Interactive Graph Search with Bounded}

In this section, we investigate the categorization problem for both single and multiple target. We propose the \single and \multi methods to find the approximate target labels with limited questions.

\begin{algorithm}[t]
  \caption{\single}
  \label{algo:single}
  \begin{algorithmic}[1]
    \Require A hierarchy tree $T=(V, E, \pr)$, a root $r$, a budget number $B$.
    \Ensure A target label $x$.
    \State Let $\val(V) \leftarrow \pr(V)$;
    \State Let $\can \leftarrow V$;
    \For {$i \leftarrow$ 1 to $B$}
      \For {$v \in \can \setminus Y$}
        \State $\pyes(v) = \sum_{u \in \des(v)}{\pr(u)}, \pno(v) = 1 - \pyes(v)$;
        \State $\cyes \leftarrow \can \cap \des(v), \cno \leftarrow \can \setminus \des(v)$;
        \State $\gyes(v) = \sum_{u \in \cyes}{\dist \langle v, u \rangle \cdot \val(u)}$;
        \State $\gno(v) = \sum_{u \in \cno}{\dist \langle r, u \rangle \cdot \val(u)}$;
      \EndFor
      \State $v^* = \arg\min_{v \in V \setminus N} {\gyes(v) \cdot \pyes(v) + \gno(v) \cdot \pno(v)}$;
      \State $ANS \leftarrow question(v^*)$;
      \If {$ANS = \yes$}
        \State $\can^* \leftarrow \can \cap \des(v^*)$;
        \State $r \leftarrow v^*$;
      \Else
        \State $\can^* \leftarrow \can \setminus \des(v^*)$;
      \EndIf
      \For {$u \in \can \setminus \can^*$}
        \State $\pr(u) = 0$;
      \EndFor
      \For {$u \in \can$}
        \State $\pr(u) = \pr(u) \cdot \frac{|\can|}{|\can^*|}$;
      \EndFor
      \State $\can \leftarrow \can^*$;
      \If {$\can = \{r\}$}
        \State \Return{$r$};
      \EndIf
    \EndFor
    \State \Return{$r$}; 
  \end{algorithmic}
\end{algorithm}

\subsection{Overview}

\stitle{Single-target interactive graph search.} Given a hierarchical \DAG $G = (V, E, Pr)$, which has a unique root $r$. An adversary choose arbitrary a target vertex $t$. An algorithm's goal is finding the closest label vertex $x \in Y$, i.e. $x = \arg \min_{x \in Y}{\dist \langle x, t \rangle}$, with $B$ interactive questions budget. 

\stitle{Overview.} 

\subsection{STIGS Algorithm}

\stitle{Probability calculation.} In the paper \cite{li2020efficient}, Li et al. propose the probability distribution for single target. The yes probability for each vertex $V$ follows $\pyes(v) = \sum_{u \in \des(v)}{\pr(u)}$ and no probability follows $\pno(v) = 1 - \pyes(v)$. The sum probability of all vertices equals $1$. 

Based on the probability distribution, we propose an equation to update probability after each question as follows:
\begin{equation} \label{eq.prob}
\pr(u) = 
\left\{
\begin{aligned}
&\pr(u) \cdot \frac{|\can|}{|\can^*|}, \ &u \in \can^*\\
&0, \ &u \notin \can^* \\
\end{aligned}
\right.
\end{equation}
where $N$ is the no set before question and $N^*$ is the no set after question. The general idea is that assign the probability of impossible vertices to the possible vertices and keep the sum probability equals $1$.

\stitle{Summary score.} Because of the single target, the yes set only includes all the ancients of the deepest vertex whose answer is \yes. So, the selected vertex must be the deepest \yes vertex because it is closest to the target. So, we define the summary score function $\g(Y, V \setminus N, 1) = \sum_{u \in V \setminus N}{\dist \langle v, u \rangle \cdot \val(u)}$, where $v$ is the deepest vertex in the yes set $Y$. Its meaning is to select the best vertex from yes set Y to summarize all the possible vertices in $V \setminus N$. 

\stitle{STIGS algorithm.} Based on the greedy strategy and the probability distribution, we propose an efficiency strategy to find the approximate target. Algorithm~\ref{algo:single} shows the pseudo code of \single algorithm. First, the algorithm initialize \val as the probability \pr and the set \can as vertices set (lines 1-2). Then, for each question, algorithm~\ref{algo:single} calculates the yes\&no probability (lines 5-6) and summary score in yes\&no cases (lines 7-10) for all candidate targets. Note that all these probabilities and summary scores will take totally $O(n)$ time by Depth-First Search(DFS) in tree. Next, the algorithm will choose the optimal target $v^*$ and question it (lines 11-12). For different answers, it will update the candidate set $\can$, the root vertex $r$ and probability (lines 13-22). If the answer is \yes, it will intersect the candidate set $\can$ with $\des(v^*)$, otherwise it will minus $\can \cap \des(v^*)$ (lines 13-17). The probability will be updated following the equation~\ref{eq.prob} (lines 18-21). Finally, if the root vertex $r$ is the only element left in candidate set, the algorithm will return $r$ as the exact answer (lines 23-24). Otherwise, it return $r$ after $B$ rounds of questions (line 25).

\stitle{Complexity analysis.} The algorithm should wait the crowd to return the answer, so we only consider the time complexity for each question. For the summary score calculation, the time complexity is totally $O(n)$ time by Depth-First Search(DFS) in tree cases and $O(n^2)$ time in \DAG cases. The update of no set and probability also takes $O(n)$ time. So, the time complexity of each question is $O(n)$ in tree cases and $O(n^2)$ in \DAG.

\subsection{MTIGS Algorithm}

\begin{algorithm}[t]
  \caption{\multi}
  \label{algo:multi}
  \begin{algorithmic}[1]
    \Require A hierarchy tree $T=(V, E, \pr)$, a budget number $B$, a selection number $k$.
    \Ensure A set of at most $k$ labels $S$.
    \State Let $\val(V) \leftarrow \pr(V)$;
    \State Let $\Syes \leftarrow \{r\}, \can \leftarrow V$;
    \For {$i \leftarrow$ 1 to $B$}
      \For {$v \in \can$}
        \State $\pno(v) = \prod_{u \in \des(v) \cap \can}{(1 - \pr(u))}$;
        \State $\pyes(v) = 1 - \pno(v)$;
        \State $\cyes \leftarrow \can \setminus (\can \cap (\anc(v) \setminus \{v\}))$;
        \State $\cno \leftarrow \can \setminus (\can \cap \des(v))$;
        \State $\gyes(v) = \g(\Syes \cup \anc(v), \cyes, k)$;
        \State $\gno(v) = \g(\Syes, \cno, k)$;
      \EndFor
      \State $v^* = \arg\min_{v \in V \setminus N} {\gyes(v) \cdot \pyes(v) + \gno(v) \cdot \pno(v)}$;
      \State $ANS \leftarrow question(v^*)$;
      \If {$ANS = \yes$}
        \State $\Syes \leftarrow \Syes \cup \anc(v^*)$;
        \State $\can^* \leftarrow \can \setminus (\can \cap (\anc(v^*) \setminus \{v^*\})$;
      \Else
        \State $\can^* \leftarrow \can \setminus (\can \cap \des(v^*))$;
      \EndIf
      \For {$u \in \can \setminus \can^*$}
        \State $\pr(u) = 0$;
      \EndFor
      \State $\can \leftarrow \can^*$;
      \If {$\can \subseteq \Syes$}
        \State \textbf{break};
      \EndIf
    \EndFor
    \State $S^* = \arg \min_{S \subseteq \Syes, |S| \leq k}{\g(S, \can)}$;
    \State \Return{$S^*$}; 
  \end{algorithmic}
\end{algorithm}

\stitle{STIGS algorithm.} Based on the greedy strategy and the probability distribution, we propose an efficiency strategy to find the approximate target. Algorithm~\ref{algo:single} shows the pseudo code of \single algorithm. First, the algorithm initialize \val as the probability \pr and the set \can as vertices set (lines 1-2). Then, for each question, algorithm~\ref{algo:single} calculates the yes\&no probability (lines 5-6) and summary score in yes\&no cases (lines 7-10) for all candidate targets. Note that all these probabilities and summary scores will take totally $O(n)$ time by Depth-First Search(DFS) in tree. Next, the algorithm will choose the optimal target $v^*$ and question it (lines 11-12). For different answers, it will update the candidate set $\can$, the root vertex $r$ and probability (lines 13-22). If the answer is \yes, it will intersect the candidate set $\can$ with $\des(v^*)$, otherwise it will minus $\can \cap \des(v^*)$ (lines 13-17). The probability will be updated following the equation~\ref{eq.prob} (lines 18-21). Finally, if the root vertex $r$ is the only element left in candidate set, the algorithm will return $r$ as the exact answer (lines 23-24). Otherwise, it return $r$ after $B$ rounds of questions (line 25).

\stitle{Complexity analysis.} The algorithm should wait the crowd to return the answer, so we only consider the time complexity for each question. For the summary score calculation, the time complexity is totally $O(n)$ time by Depth-First Search(DFS) in tree cases and $O(n^2)$ time in \DAG cases. The update of no set and probability also takes $O(n)$ time. So, the time complexity of each question is $O(n)$ in tree cases and $O(n^2)$ in \DAG.

\subsection{Summary Algorithm}


